SinReQ: Generalized Sinusoidal Regularization for Low-Bitwidth Deep Quantized Training

Deep quantization of neural networks (below eight bits) offers significant promise in reducing their compute and storage cost. Albeit alluring, without special techniques for training and optimization, deep quantization results in significant accuracy loss. To further mitigate this loss, we propose a novel sinusoidal regularization, called SinReQ1, for deep quantized training. SinReQ adds a periodic term to the original objective function of the underlying training algorithm. SinReQ exploits the periodicity, differentiability, and the desired convexity profile in sinusoidal functions to automatically propel weights towards values that are inherently closer to quantization levels. Since, this technique does not require invasive changes to the training procedure, SinReQ can harmoniously enhance quantized training algorithms. SinReQ offers generality and flexibility as it is not limited to a certain bitwidth or a uniform assignment of bitwidths across layers. We carry out experimentation using the AlexNet, CIFAR-10, ResNet-18, ResNet-20, SVHN, and VGG-11 DNNs with three to five bits for quantization and show the versatility of SinReQ in enhancing multiple quantized training algorithms, DoReFa [32] and WRPN [24]. Averaging across all the bit configurations shows that SinReQ closes the accuracy gap between these two techniques and the full-precision runs by 32.4% and 27.5%, respectively. That is improving the absolute accuracy of DoReFa and WRPN by 2.8% and 2.1%, respectively.

==> body/ablation_studies.tex <==
\section{Ablation Studies and Discussion}
% (add something?)
\subsection{Influence of Reward Function}\label{sec:reward}
%
The design of reward function is a crucial component of reinforcement learning as indicated in section \ref{sec:Reward}.
%
There are many possible reward functions one could define for a particular application setting. However, different designs could lead to either different policies or different convergence behavior.
%
In this paper, we incorporate reward engineering by proposing special parametric reward formulation. First, we argue that the proposed formulation helps to achieve better final performance during fixed amount of training episodes (performance here can be interpreted either as better final solution quality or faster convergence time). Second, in this context of multi-objective optimization, where there are a set of optimal solutions (defined by the Pareto frontier), the actual cost-benefit tradeoff (accuracy state vs quantization state) is controlled by having a parametric formulation.
%
To evaluate the effectiveness of the proposed reward formulation, we have compared three different reward formulations: $(i)$ proposed in section \ref{sec:Reward}, $(ii) R=acc_st/quant_st$, $(iii) R=acc_st-quant_st$. Figure \ref{fig:diff_rewards} summarizes the convergence behavior for the three formulations. 
%
The proposed reward formulation consistently shows higher performance in terms of faster convergence time and better solution quality as compared to others.
%

\iffalse 
\subsection{Evaluation of State Embeddings}
State embeddings are an essential component in determining and controlling the convergence behavior of the RL agent. We carried out experiments to evaluate the effectiveness of the used state embeddings. In every iteration, we repeat the same experiment while omitting one state embedding at a time and keeping the rest. Based on our experiments, we observe that the layer's size/dimensions turn out to be the most important embedding for convergence. Standard deviation of the layer's weights comes as the second most important parameter. Figure \ref{fig:wo-weight-stat} shows convergence behavior for LeNet with variance of weights as part of the state embedding (baseline result) and Figure \ref{fig:w-weight-stat} shows the behavior when variance of weights was excluded from the state embedding. The rest of the state embeddings help in speeding up the convergence process.
%
\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/probs-wo-weight-stats}
  \caption{Excluding weight variance in the state embedding}
    \label{fig:wo-weight-stat}
\end{subfigure}
%
\begin{subfigure}{0.4\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/probs-w-weight-stats}
  \caption{Including weight variance in the state embedding}
    \label{fig:w-weight-stat}
\end{subfigure}
\caption{Comparison of ReLeQ convergence performance for LeNet (convolution layer 1) on MNIST dataset (a) when weight variances are excluded from the state embedding and (b) when weight variances are included in the state embedding	.}
\label{fig:weight_stats}
\end{figure}
%
\fi

\subsection{Tuning PPO clipping parameter}\label{sec:clipping_param_tuning}
One of the unique features about PPO algorithm is its novel objective function with clipped probability ratios, which forms a pessimistic estimate
(i.e., lower bound) of the performance of the policy. Such modification restricts the range that the new policy can vary from the old one, hence improves the stability of the learning process.  With Clipped Surrogate Objective function, we have two probability ratios, one non clipped and one clipped in a range between $\lbrack1-\epsilon$, $1+\epsilon\rbrack$, where $\epsilon$ is a hyper parameter that helps to define this clip range. Table \ref{table:clipping_table} provides a summary of tuning epsilon (commonly in the range of 0.1, 0.2, 0.3). Based on our performed experiments, $\epsilon=0.1$ often reports the highest average reward across different benchmarks.


==> body/background.tex <==
%\section{Background}
%\subsection{Deep Reinforcement Learning}
%Recent advancements in combining deep learning techniques with reinforcement learning have led to phenomenal feats like Deepmind's AlphaZero which learns to play with zero human intervention and OpenAI Five, a team of five networks which has been defeating human teams in Dota 2. While deep learning enables us to understand unstructured environments, reinforcement learning provides a formalism for behavior and both of these combined allow us to solve much more complex problems in an unsupervised environment. Neural Fitted Q Learning (NFQ) was one of the first efforts in combining these two fields but the major breakthrough in Deep Reinforcement Learning was with introduction of Deep Q-Networks(DQNs), which could master a diverse set of Atari games and surpass human performance. And from that point on, improvements in DQNs and new methods such as Policy Gradients have accelerated the progress in Deep Reinforcement Learning.
%
%\subsection{Proximal Policy Optimization}\label{sec:PPO}
%
%Policy Gradient Methods have played central part in the recent breakthroughs in Deep Reinforcement Learning and these algorithms aim to address some of the disadvantages of using value based methods (DQNs) like big oscillations while training, inefficiency in handling large action spaces and the inability to learn stochastic policies. We use Proximal Policy Optimization(PPO), which is the state-of-the art algorithm based on Policy Gradient Method to train our RL agent. While most standard policy gradient algorithms perform only one gradient update per batch, PPO enables multiple epochs of updates per batch. PPO also avoids too large policy updates by clipping the probability ratios between old and new policies to the range of 0.8 to 1.2.
%
%\subsection{Related Work}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/block_diagram_2.pdf}
    \caption{Overview of ReLeQ framework.}		  
    \label{fig:block_diagram}
%    \vspace{0.2cm}
\end{figure*}


==> body/experimental_setup.tex <==
\section{Experimental Setup}
\vspace{-3ex}
\label{sec:exp}
 \begin{table}[!h]
	\centering
	\caption{Benchmark DNNs and their deep quantization with \releq.}
	\includegraphics[width=0.95\linewidth]{figs/results_summary_table.pdf}
	\label{table:networks}
	\vspace{-0.5cm}
\end{table}
%
\vspace{-0.2cm}
\paragraph{Benchmarks.}
%
To assess the effectiveness of \releq across a variety of DNNs, we use the following seven diverse networks that have been used in different real-world vision tasks: AlexNet, CIFAR-10 (simplenet), LeNet, MobileNet (Version 1), ResNet-20, SVHN and VGG-11.
%
Of these seven networks, AlexNet and MobileNet were evaluated on the ImageNet (ILSVRC'12) dataset, ResNet-20, VGG-11 and CIFAR-10 on CIFAR-10, SVHN on SVHN  and LeNet on the MNIST dataset.  

\vspace{-0.2cm}
\paragraph{Quantization technique.} We use the technique proposed in WRPN \cite{Mishra2017WRPNWR} where weights are first scaled and clipped to the $(-1.0, 1.0)$ range and quantized as per the following equation. 
%
The term $k$ is the bitwidth used for quantization out of which $k-1$ bits are used for quantization and one bit is used for sign.
%
\begin{small}
\vspace{-2ex}
	$$ x_{q} = \frac{round((2^{k-1} - 1)x_{f})}{2^{k-1} - 1}$$
	\vspace{-3ex}
\end{small}

\vspace{-0.5cm}
\paragraph{Deep quantization with conventional hardware.} \releq's solution can be deployed on conventional hardware, such as general purpose CPUs to provide benefits and improvements. 
%
To manifest this, we have evaluated \releq using TVM~\cite{TVM} on an Intel Core i7-4790 CPU.
%
We use TVM since its compiler supports deeply quantized operations with bit-serial vector operations on conventional hardware. 
%
We compare our solution in terms of the inference execution time (since the TVM framework does not offer energy measurements) against 8-bit quantized network. 
%
The results can be seen in Figure~\ref{fig:tvm} and will be further elaborated in the next section.

\vspace{-0.5cm}
\paragraph{Deep quantization with custom hardware accelerators.} To further demonstrate the energy and performance benefits of the solution found by \releq, we evaluate it on Stripes~\cite{stripes}, a custom accelerator designed for DNNs, which exploits bit-serial computation to support flexible bitwidths for DNN operations
%
Stripes does not support or benefit from deep quantization of activations and it only leverages the quantization of weights. 
%
We compare our solution in terms of energy consumed and inference execution time against the 8-bit quantized network.

\vspace{-0.5cm}
\paragraph{Comparison with prior work.} 
%
We also compare against prior work~\cite{Ye2018AUF}, which proposes an iterative optimization procedure (dubbed ADMM) through which they find quantization bitwidths only for AlexNet and LeNet. 
%
Using Stripes~\cite{stripes} and TVM~\cite{TVM}, we show that \releq's solution provides higher performance and energy benefits compared to ADMM~\cite{Ye2018AUF}. 
%

\begin{table}
	\centering
	\caption{Hyper-Parameters of PPO used in ReLeQ.}
	
	\includegraphics[width=0.95\linewidth]{figs/hyperparam_table.pdf}
	\label{table:ppo_params}
	\vspace{-0.5cm}
\end{table}

\vspace{-0.5cm}
\paragraph{Implementation and hyper-parameters of the Proximal Policy Optimization (PPO).}
%
As discussed, \releq use PPO~\cite{ppo} as its RL engine, which we implemented in python where its policy and value networks use TensorFlow's Adam Optimizer with an initial learning rate of $10^{-4}$. 
%
The setting of the other hyper-parameters of PPO is listed in Table~\ref{table:ppo_params}.




==> body/learning_proc.tex <==
 
\section{Putting it All Together: \releq in Action}
\label{sec:releq_working}
\vspace{-1ex}

%
As discussed in Section~\ref{sec:rl_quantization}, state, action and reward enable the \releq agent to maneuver the search space with an objective of quantizing the neural network with minimal loss in accuracy.
%
\releq starts with a pretrained model of full precision weights and proposes quantization levels of weights for all layers in a DNN.
%
Figure~\ref{fig:overview} depicts the entire workflow for \releq and this section gives an overview of how everything fits together.

\niparagraph{Interacting with the environment.}
%
\releq agent steps through all layers one by one, determining the quantization level for the layer at each step.
%
For every step, the state embedding for the current layer comprising of different elements described in Section~\ref{sec:state} is fed as an input to the Policy and Value Networks of the \releq agent and the output is the probability distribution over the different possible bitwidths and value of the state respectively.
%
\releq agent then takes a stochastic action based on this probablity distribution and chooses a quantization level for the current layer.
%
Weights for this particular layer are quantized to the predicted bitwidth and  with accuracy preservation being a primary component of \releq's reward function, retraining of a quantized neural network is required in order to properly evaluate the effectiveness of deep quantization.
%
Such retraining is a time-intensive process and it undermines the search process efficiency.
%
To get around this issue, we reward the agent with an estimated validation accuracy after retraining for a shortened amount of epochs.
%
For deeper networks, however, due to the longer retraining time, we perform this phase after all the bitwidths are selected for the layers and then we do a short retraining.
%
Dynamic network specific parameters listed in Table~\ref{table:state_embed} are updated based on the validation accuracy and current quantization levels of the entire network before stepping on to the next layer.
%
In this context, we define an epsiode as a single pass through the entire neural network and the end of every episode, we use Proximal Policy Optimization~\cite{ppo} to update the Policy and Value networks of the \releq agent.
%
After the learning process is complete and the agent has converged to a quantization level for each layer of the network, for example 2 bits for second layer, 3 bits for fourth layer and so on, we perform a long retraining step using the quantized bitwidths predicted by the agent and then obtain the final accuracy for the quantized version of the network.
%
%To encourage lower bitwidth quantization, the RL agent factors the average quantization across all layers into the reward in combination with the aforementioned retrained accuracy.
%
%A positive accuracy reward is determined by an improved or maintained validation accuracy relative to the full precision accuracy, wh ereas the quantization reward is positive if the agent reduces the bitwidth of a layer.
%
%The interplay between accuracy reward and quantization reward enables the agent to deeply quantize the network with minimal loss in accuracy.
% 
%

\niparagraph{Learning the Policy.}
%
Policy in terms of neural network quantization is to learn to choose the optimal bitwidth for each layer in the network.
%
Since \releq uses a Policy Gradient based approach, the objective is to optimize the policy directly, it's possible to visualize how policy for each layer evolves with respect to time i.e the number of episodes.
%		
Figure \ref{fig:releq_lenet_policy} shows the evolution of \releq agent's bitwidth selection probabilities for all layers over time (number of episodes), which reveals how the agent's policy changes with respect to selecting a bitwidth per layer. As indicated on the graph, the end results suggest the following quantization patterns, ${2, 2, 2, 2}$ or ${2, 2, 3, 2}$ bits. 
For the first two convolution layers (Convolution Layer 1, Convolution Layer 2), the agent ends up assigning the highest probability for two bits and its confidence increases with increasing number of training episodes.
%
For the third layer (Fully Connected Layer 1), the probabilities of two bits and three bits are very close. Lastly, for the fourth layer (Fully Connected Layer 2), the agent again tends to select two bits, however, with relatively smaller confidence compared to layers one and two.
%
With these observations, we can infer that bitwidth probability profiles are not uniform across all layers and that the agent distinguishes between the layers, understands the sensitivity of the objective function to the different layers and accordingly chooses the bitwidths.
%
%The 4 design points highlighted in black, however, could be considered as outliers since each one of them has at least one layer with a bitwidth=1. In general, using bitwidth=1 for this network relapses the accuracy, except for these 4 special combinations. We posit this as a possible reason that the RL agent did not have this in its policy since it is not a consistent rule or behavior to learn. \\
%
Looking at the agent's selection for the third layer (Fully Connected Layer 1) and recalling the initial problem formulation of quantizing all layers while preserving the initial full precision accuracy, it is logical that the probabilities for two and three bits are very close. Going further down to two bits was beneficial in terms of quantization while staying at three bits was better for maintaining good accuracy which implies that third layer precision affects accuracy the most for this specific network architecture. \textit{This points out the importance of tailoring the reward function and the role it plays in controlling optimization tradeoffs}.

==> body/methodology.tex <==
\section{Our Method: Quantization Friendly Regularization Technique}
\label{sec:method}
\vspace{-1ex}

%
The most commonly used regularization technique is known as \textit{weight decay}, which aims to reduce the network complexity by limiting the growth of the weights. It is realized by adding a term to the objective function that penalizes large weight values 
%\cite{Krogh:1991:SWD:2986916.2987033}:
\[ E(w) = E_o(w) + \frac{1}{2} \lambda \sum\limits_{i} {w_i}^2 \]
where $E_o$ is the original loss measure, and $\lambda$ is a parameter governing how strongly large weights are penalized. $w$ is a vector containing all free parameters of the network.
%
\begin{figure}[t]
	\centering
	\subfloat[t][]{\includegraphics[width=0.35\textwidth]{figs/quant_friendly_a.pdf}
		\label{fig:quant_a}}
	\subfloat[t][]{\includegraphics[width=0.29\textwidth]{figs/quant_friendly_b.pdf}
		\label{fig:quant_b}}
	\subfloat[t][]{\includegraphics[width=0.25\textwidth]{figs/quant_friendly_c.pdf}
		\label{fig:quant_c}}
	\caption{Quantization friendly regularization.}
	\label{fig:sin2_reg}
\end{figure}
\subsection{Periodic Regularization}
%
{\setlength{\parindent}{0cm}Here, we propose a new type of regularization that is friendly to quantization. 
%
The proposed regularization is realized by adding a periodic function (regularizer) to the original objective function, Figure \ref{fig:quant_a}. 
%
The periodic regularizer has a periodic pattern of minima that correspond to the desired quantization levels. Such correspondence is achieved by matching the period to the quantization step based on a particular number of bits for a given layer.}
%\[ E(w) = E_o(w) + \frac{1}{2} \lambda_{q} \sum\limits_{i} {\sin^{2}\left({\frac {\pi w_i} {2^{-qbits}}}\right)} \]
\[ E(w) = E_o(w) + \frac{1}{2} \lambda \sum\limits_{i} {w_i}^2 + \frac{1}{2} \lambda_{q} \sum\limits_{i} {\sin^{2}\left({\frac {\pi w_i} {2^{-qbits}}}\right)} \]
where $E_o$ is the original loss measure, and $\lambda_q$ is a parameter governing how strongly weight quantization errors are penalized. $w$ is a vector containing all free parameters of the network.
%
For the sake of simplicity and clarity, Figures \ref{fig:quant_b} and \ref{fig:quant_c} depict a geometrical sketch for a hypothetical loss surface (original objective function to be minimized) and an extra regularization term in 2-D weight space. 
%
For weight decay regularization, in Figure \ref{fig:quant_b}, the faded circular contours show that as we get closer to the origin, the regularization loss is minimized. Optimum solution is achieved by striking a balance between the original loss term and the regularization loss term.
%
In a similar way, Figure \ref{fig:quant_c} shows a representation of the proposed regularization. A periodic pattern of minima pockets is seen surrounding the original optimum point. 
%
The objective of the optimization problem is to find the best solution that is the closest to one of those minima pockets where weight values are nearly matching the desired quantization levels, hence the name quantization-friendly.
%


==> body/outline.tex <==
\section{RELEQ for large networks}

- 
%
\begin{itemize}
	\item Table.1  Results: layers weights quantization bitwidths for AlexNet and Resnet-20
	\item Sub-section: Algorithmic Changes (moving from small networks to large networks) Reward per network / reward 			boosting / normalization techniques (mathematical formulas)
	\item Fig.1  Policy evolution (quantization bitwidths probability profiles)
	\begin{itemize}
    		\item X-axis: number of episodes 
	        \item 	Y-axis: selection probability 
        	        \item (a) Without Algorithmic changes for Resnet-20 (divergence behavior, oscillations)
	        \item	(b) With Algorithmic changes for Resnet-20 (convergence)
   	\end{itemize}
\end{itemize}

%
\section{Computation Cost}
\begin{itemize}
\item Sub-section: modified RELEQ formulation; replacing quantization state to computation state
\item Table.1: Results: layers weights quantization bitwidths for AlexNet and Resnet-20 (comparing results (bitwidths) with quantization state vs with computation state. Basically showing how the suggested bitwidths would change considering per layer computation cost into account)
\end{itemize}

%
\section{Proposed new regularization technique (quantization-friendly)}


\begin{itemize}
	\item Sub-section: High level idea / theory / mathematical formulation [DONE]
	\item Fig.1: High level idea / theory [DONE]
	\item Fig.2: Accelerated fine-tuning Results (with and without proposed regularization) 
		Benchmark: CIFAR10 [DONE]
	\item Fig.3: (histogram) Weights evolution towards quantized levels during fine-tuning. For example: 
	\begin{itemize}
    		\item X-axis: weights numerical values 
	        \item 	Y-axis: number of occurrences 
        	        \item (a) Original weight distribution for a particular layer 
	        \item (b) Weights distribution after epoch1 (midway of finetuning)
	        \item (c) Weights distribution after epoch2 or end of finetuning (weights are clustered around quantized levels)
   	\end{itemize}
\end{itemize}




==> body/outlook.tex <==
\section{Accelerated Finetuning}
%
 %\niparagraph{Loss function of neural networks.}
 \paragraph{Loss function of neural networks.}
 %
 Neural networks' loss functions are known to be highly non-convex and generally very poorly understood. It has been empirically verified that loss surfaces for large neural networks have many local minima that are essentially equivalent in terms of test error \cite{DBLP:journals/corr/ChoromanskaHMAL14}, \cite{DBLP:journals/corr/abs-1712-09913}. 
%
Moreover, converging to one of the many good local minima proves to be more useful as compared to struggling to find the global minimum of the accuracy loss on the training set (which often leads to overfitting). This opens up and encourages a possibility of adding extra custom objectives to optimize for (during the training process), in addition to the original one (accuracy loss). The added custom objective could be with the purpose of increasing generalization performance or imposing some preference on the weights values. 
%
Regularization is one of the major techniques that makes use of such facts as discussed in the following subsection.
 
 %


%\niparagraph{Quantization friendly regularization.}
\paragraph{Quantization friendly regularization.}
%
Neural networks often suffer from redundancy of parameterization and consequently they commonly tend to overfit.
%
Regularization is one of the commonly used techniques to enhance generalization performance of neural networks.
%
Regularization effectively constrains weight parameters by adding a term (regularizer) to the objective function that captures the desired constraint in a soft way. This is achieved by imposing some sort of preference on weights updates during the optimization process. As a result, regularization seamlessly leads to unconditionally constrained optimization problem instead of explicitly constrained which, in most cases is much more difficult to solve.
%
The most commonly used regularization technique is known as \textit{weight decay}, which aims to reduce the network complexity by limiting the growth of the weights. It is realized by adding a term to the objective function that penalizes large weight values \cite{Krogh:1991:SWD:2986916.2987033}:
\[ E(w) = E_o(w) + \frac{1}{2} \lambda \sum\limits_{i} {w_i}^2 \]

where $E_o$ is the original loss measure, and $\lambda$ is a parameter governing how strongly large weights are penalized. $w$ is a vector containing all free parameters of the network.
%

%\begin{figure}[t]
%	\centering
%	\subfloat[t][]{\includegraphics[width=0.35\textwidth]{figs/quant_friendly_a.pdf}
%		\label{fig:quant_a}}
%	\subfloat[t][]{\includegraphics[width=0.29\textwidth]{figs/quant_friendly_b.pdf}
%		\label{fig:quant_b}}
%	\subfloat[t][]{\includegraphics[width=0.25\textwidth]{figs/quant_friendly_c.pdf}
%		\label{fig:quant_c}}
%	\caption{Quantization friendly regularization.}
%	\label{fig:sin2_reg}
%\end{figure}



\begin{figure}[t]
\centering
\begin{subfigure}{0.35\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_a.pdf}
		\caption{some caption}
		\label{fig:quant_a}
\end{subfigure}

\begin{subfigure}{0.29\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_b.pdf}
	\caption{some caption}
		\label{fig:quant_b}
\end{subfigure}

\begin{subfigure}{0.25\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_c.pdf}
  \caption{some caption}
	\label{fig:quant_c}
\end{subfigure}
\caption{Quantization friendly regularization.}
\label{fig:sin2_reg}
\end{figure}


{\setlength{\parindent}{0cm}Here, we propose a new type of regularization that is friendly to quantization. The proposed regularization is realized by adding a periodic function (regularizer) to the original objective function, Figure \ref{fig:quant_a}. The periodic regularizer has a periodic pattern of minima that correspond to the desired quantization levels. Such correspondence is achieved by matching the period to the quantization step based on a particular number of bits for a given layer.}
\[ E(w) = E_o(w) + \frac{1}{2} \lambda_{q} \sum\limits_{i} {\sin^{2}\left({\frac {\pi w_i} {2^{-qbits}}}\right)} \]
where $E_o$ is the original loss measure, and $\lambda_q$ is a parameter governing how strongly weight quantization errors are penalized. $w$ is a vector containing all free parameters of the network.
%

For the sake of simplicity and clarity, Figures \ref{fig:quant_b} and \ref{fig:quant_c} depict a geometrical sketch for a hypothetical loss surface (original objective function to be minimized) and an extra regularization term in 2-D weight space. 
For weight decay regularization, in Figure \ref{fig:quant_b}, the faded circular contours show that as we get closer to the origin, the regularization loss is minimized. Optimum solution is achieved by striking a balance between the original loss term and the regularization loss term.
%
In a similar way, Figure \ref{fig:quant_c} shows a representation of the proposed regularization. A periodic pattern of minima pockets is seen surrounding the original optimum point. The objective of the optimization problem is to find the best solution that is the closest to one of those minima pockets where weight values are nearly matching the desired quantization levels, hence the name quantization-friendly.
%

%\niparagraph{Evaluation.}
\paragraph{Evaluation.}
%
To demonstrate the effectiveness of the proposed regularization, Figure \ref{fig:sin2_eval_1} shows a comparison of the validation accuracy for CIFAR-10 using conventional finetuning approach versus finetuning with the proposed approach. It can be noticed that, under same limited amount of retraining steps, medium number of bits seem to benefit the most. Observed performance improvements could differ across different networks and different durations of retraining.
%
It should be noted that, using the proposed regularization approach, the weight updates occur in full precision as opposed to clipping the weights to the quantized values, yet the weights eventually converge to desired quantization levels.
 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/val_accuracy.pdf}
    \caption{Comparison of validation accuracy of CIFAR-10 after retraining for 10k steps at different quantization bitwidths for weights (assuming same bitwidth for all layers).}		  
    \label{fig:sin2_eval_1}
    \vspace{0.2cm}
\end{figure}




==> listings/algorithm.tex <==
%\begin{algorithm}
%\caption{Reward Formulation}
\vspace{-12pt}
\begin{algorithmic}
\STATE \textbf{\underline{Reward Shaping:}}
%\STATE $ reward = 1 - (State_{Quantization})^a $ 
\STATE $ reward = 1.0 - (State_{Quantization})^a $ 
%\IF{$(State_{Accuracy} < threshold) $}
\IF{$(State_{Accuracy} < th) $}
	\STATE {$reward = -1.0 $}
\ELSE
	\STATE $Acc_{discount} = max(State_{Accuracy}, th)^{(b/max(State_{Accuracy}, th))}$ 
	\STATE $reward = reward \times Acc_{discount}$ 
\ENDIF 
\end{algorithmic}
%\end{algorithm}
\vspace{0pt}

